Transferability Through Cooperative Competitions

This paper presents a novel framework for cooperative robotics competitions (coopetitions) that promote the transferability and composability of robotics modules, including software, hardware, and data, across heterogeneous robotic systems. The framework is designed to incentivize collaboration between teams through structured task design, shared infrastructure, and a royalty-based scoring system. As a case study, the paper details the implementation and outcomes of the first euROBIN Coopetition, held under the European Robotics and AI Network (euROBIN), which featured fifteen robotic platforms competing across Industrial, Service, and Outdoor domains. The study highlights the practical challenges of achieving module reuse in real-world scenarios, particularly in terms of integration complexity and system compatibility. It also examines participant performance, integration behavior, and team feedback to assess the effectiveness of the framework. The paper concludes with lessons learned and recommendations for future coopetitions, including improveme

==> results_aux.tex <==
% SRL Results
Starting by addressing the task conditional levels, most teams ended up changing their initial Pick Location $L_{i}$ (50\% to 70\% of teams) accross tasks. Some teams also changed their Object $O_{i}$ (25\% to 35\% of teams), and, although less common, they also changed their Place Location $L_{j}$ (15\% of teams).

Focusing on Task #1 where teams had to operate in their chosen \textbf{base kitchen}, teams struggled for the most part in milestones 5 and 6, where they were expected to open the drawer/cabinet/dishwasher and detect the request object, as illustrated in figure \ref{fig:wp2-results}.

On the milestone conditional level side, most teams did the navigation milestones autonomously apart from two teams which used teleoperation. The command understading was done via speech accross teams, as for the object detection, teams opted for several different objects present in the pick location without any occlusions from the robot's point of view (POV).

Regarding manipulation, some teams required human assistance, other used teleoperation, and others did it fully autonomously without the need for custom handles.

Looking at penalties, minor instances of robot collisions during navigation and manipulation milestones took place. On the subjective score side, the judges evaluated teams on different scales as depicted in figure \ref{fig:wp2-results}. This assement can be correlated with teams options on milestone conditional levels, which teams opted for simpler approaches, e.g artifical landmarks or teleoperation, rather than fully autonomous behaviours expected by these external referees.

About the transferability, the Pinocchio Library, and the LLM Task Planning modules have been used accross miletones as illustrated by figure \ref{fig:wp2-results}. Data modules such as the shared table obj file had also been useful in most milestones. Other modules such as the HappyPose, and Speech-To-Text and Text-To-Speech modules have been used in the perception and comand understading milestones.

==> wp1_aux.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Industrial Robots League, skills description table
% Status: not used
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table}[h]
%\centering
%\vspace{10pt}  % Adds vertical space between "Table 1" and the table
%\begin{tabular}{|m{8em}|m{6cm}|}
%\hline
%\rowcolor[HTML]{cc7d7a}
%\multicolumn{1}{|c|}{\textbf{Skill Category}} & \multicolumn{1}{c|}{\textbf{Description}} \\ \hline
%Object Localization & Robot must detect the location of the task board and press a button. \\ \hline
%Interactive Manipulation & Robot must read a randomly generated setpoint value from a screen and move a slider to match. \\ \hline
%Insertion & Robot must pick up the Probe Plug and insert it into the Test Port. \\ \hline
%Levering & Robot must open the hinged door, pick up the Probe, and insert it into the terminal block. \\ \hline
%Wrapping & Robot must wrap the cable of the Probe around two posts and insert the Probe back into its holder. \\ \hline
%Pressing & Robot must press a button to end the trial. \\ \hline
%\end{tabular}
%\vspace{10pt}  % Adds vertical space between the table and the caption
%\caption{The manipulation skills and capabilities under examination in the Industrial Robot League.}
%\label{fig:wp1_functionalities_table}
%\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Industrial Robots League, tables scores
% Status: not used
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%
% Task milestones
%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
\vspace{10pt}
\begin{tabular}{|c|c|c|}
\hline
\rowcolor[HTML]{cc7d7a}
\textbf{Milestone} & \textbf{Task Description} & \textbf{Score} \\ \hline
MS\textsubscript{1} & Press blue button & 100 \\ \hline
MS\textsubscript{2} & Pick up probe plug & 100 \\ \hline
MS\textsubscript{3} & Insert probe plug & 300 \\ \hline
MS\textsubscript{4} & Reach SP1 center & 100 \\ \hline
MS\textsubscript{5} & Reach SP2 on screen & 300 \\ \hline
MS\textsubscript{6} & Open door & 200 \\ \hline
MS\textsubscript{7} & Insert probe and close circuit & 400 \\ \hline
MS\textsubscript{8} & Trigger post sensor & 400 \\ \hline
MS\textsubscript{9} & Insert probe tip into holder & 100 \\ \hline
MS\textsubscript{10} & Press stop button & 100 \\ \hline
\end{tabular}
\vspace{10pt}
\caption{Milestones scores in the Task Board Manipulation Challenge.}
\label{tab:irl_milestones_scores}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Task milestones conditional levels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
\vspace{10pt}
\begin{tabular}{|m{6cm}|m{0.4cm}|}
\hline
\rowcolor[HTML]{cc7d7a}
\textbf{Milestone Conditional Level Description} & \textbf{$l_{m}$} \\ \hline
The robot requires human assistance & 0.0 \\ \hline
The robot is teleoperated within the operator’s line of sight & 0.3 \\ \hline
Slider not actively perceived & 0.5 \\ \hline
Cable partially wrapped (only a single loop around the supports) & 0.5 \\ \hline
The robot is teleoperated from a remote location & 0.6 \\ \hline
The team attaches a custom handle to the taskboard to accommodate their specific gripper & 0.6 \\ \hline
The robot manipulator is fully autonomous and the taskboard is left unchanged & 1.0 \\ \hline
\end{tabular}
\vspace{10pt}
\caption{Milestones conditional levels in the Task Board Manipulation Challenge.}
\label{tab:irl_milestones_lm}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Task milestones conditional levels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
\vspace{10pt}
\begin{tabular}{|m{6cm}|m{0.4cm}|}
\hline
\rowcolor[HTML]{cc7d7a}
\textbf{Milestone Penalties Description} & \textbf{$p_{m}$} \\ \hline
The robot collides with the task board, table or any other object present in the environment & 100 \\ \hline
\end{tabular}
\vspace{10pt}
\caption{Milestones penalties in the Task Board Manipulation Challenge.}
\label{tab:irl_milestones_lm}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Task conditional levels
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
\vspace{10pt}
\begin{tabular}{|m{6cm}|m{0.4cm}|}
\hline
\rowcolor[HTML]{cc7d7a}
\textbf{Task Conditional Level Description} & \textbf{$T$} \\ \hline
Task board fixed within the table & 0.6 \\ \hline
Task board randomly posited within the table & 1.0 \\ \hline
\end{tabular}
\vspace{10pt}
\caption{Task conditional levels in the Task Board Manipulation Challenge.}
\label{tab:irl_milestones_lm}
\end{table}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Results}
\label{sec:results}

This section analyzes the outcomes of the first euROBIN Coopetition through the lens of module reuse and integration. Rather than focusing solely on robot performance, our emphasis is on how the coopetition framework supported the transfer of software, data, and perception modules across heterogeneous robotic platforms in real-world scenarios.

\subsection{Module Transferability Across Leagues}

The Marketplace phase resulted in the successful upload of a variety of modules, including perception tools, data resources, speech interfaces, and planning frameworks. However, actual module integration during the On-Site Coopetition revealed both the potential and limitations of current reuse practices.

\paragraph{Industrial Robots League}

In the IRL, module reuse was minimal but meaningful. The \textit{TUM Task Board Perception Package} was successfully adopted by multiple teams for perception tasks in three milestones: pressing the start button (\(MS1\)), moving sliders (\(MS4\)), and pressing the stop button (\(MS10\)). Its integration corresponded with increased success rates and higher subjective scores in those milestones.

Despite this success, no shared modules for manipulation or control were integrated. This suggests that while perception solutions with minimal platform dependencies are transferable, modules requiring tight coupling with hardware—such as those for actuation—remain difficult to generalize.

\paragraph{Service Robots League}

This league saw a broader range of module reuse. The \textit{Pinocchio Library} (kinematics), \textit{LLM-based Task Planner}, \textit{Speech-To-Text}, and \textit{Text-To-Speech} modules were integrated across teams to support planning, command understanding, and human-robot interaction. Several teams also reused a shared table mesh file (OBJ) as a data module to enhance environment awareness and simulation.

Module integration tended to concentrate around perception and planning tasks, especially in speech-based command understanding (\(MS2\)), object detection (\(MS5\)), and navigation (\(MS8\)). This league illustrated the potential of higher-level software reuse—particularly when tasks are complex and involve human interaction—but also highlighted the challenge of integrating shared manipulation modules, which were rarely adopted.

\paragraph{Outdoor Robots League}

Transferability in this league included modules supporting perception, command interpretation, and environment simulation. Notable reused modules were \textit{YOLO ROS} (parcel detection), \textit{Speech-To-Text}, and the \textit{Nancy Digital Twin}. The YOLO ROS module was used in \(MS5\) (parcel detection), while Speech-To-Text supported \(MS2\) across all tasks.

The Nancy Digital Twin module was exclusively used in \(MS1\) and \(MS3\) (navigation) of Task \#3, aiding situational planning in a complex mixed indoor/outdoor scenario.

As with the other leagues, module reuse was constrained by integration complexity and task-specific constraints. UAV teams, in particular, faced challenges in reusing modules due to strict platform-specific safety constraints.

\subsection{Cross-League Observations}

Three important patterns emerged when analyzing module transferability across all leagues:

\begin{itemize}
    \item \textbf{Perception and Speech Modules were Most Reused:} Modules for perception, language understanding, and task planning had the highest integration rates. These components typically had clear interfaces, minimal hardware assumptions, and addressed common subproblems across tasks.
    
    \item \textbf{Manipulation and Actuation Modules Were Rarely Reused:} Modules that interfaced with low-level control or required physical calibration were not widely adopted. This was due in part to hardware-specific constraints and lack of standardized interfaces.

    \item \textbf{Task Complexity Encouraged Reuse—But Only to a Point:} Teams facing more complex challenges (e.g., in Task \#3 of each league) were more likely to integrate shared modules. However, integration effort and platform compatibility remained significant bottlenecks.

\end{itemize}

These findings underscore the importance of providing reusable, well-documented, and loosely coupled modules to increase adoption. They also validate the coopetition’s role in incentivizing early adoption and reuse of general-purpose solutions.




